Episodic, compression-driven fluid venting in layered sedimentary basins

Fluid venting phenomena are prevalent in sedimentary basins globally. Offshore, these localised fluid-expulsion events are archived in the geologic record by the resulting pockmarks at the sea-floor. Venting is widely interpreted to occur via hydraulic fracturing, which requires near-lithostatic pore pressures for initiation. One common driver for these extreme pressures is horizontal tectonic compression, which pressurises the entire sedimentary column over a wide region. Fluid expulsion leads to a sudden, local relief of this pressure, which then gradually recharges through continued compression, leading to episodic venting. Pressure recharge will also occur through pressure diffusion from neighbouring regions that remain pressurised, but the combined role of compression and pressure diffusion in episodic venting has not previously been considered. Here, we develop a novel poroelastic model for episodic, compression-driven venting. We show that compression and pressure diffusion together set the resulting venting period. We derive a simple analytical expression for this venting period, demonstrating that pressure diffusion can significantly reduce the venting period associated with a given rate of compression. Our expression allows this rate of compression to be inferred from observations of episodic venting. We conclude that pressure diffusion is a major contributor to episodic fluid venting in mudstone-dominated basins.

==> Sections/Other.tex <==

\section{Levant basin}

% FEPs/Levant - explain FEPs, salt, trails, etc. and question marks about Cartwright stuff
In the eastern Mediterranean, the north Levant basin hosts over 300 fluid escape pipes which record episodic fluid venting from 13 positions across the region since 2 Ma. Within the Levant basin is a $\sim$1.5 km thick layer of salt deposited during the Messinian Salinity Crisis \citep{ryan2009decoding}. Pipes form vertically but the basinward viscous flow of salt shifts the existing pipes, requiring a replacement vertical pipe to form and vent fluid. Repetition of this process produces a linear trail of pipes \citep{cartwright2018direct}. From the spatial distributions of pockmarks from each pipe trail, the time of formation of each pipe can be estimated using the methods of \cite{oppo2021leaky} and \cite{cartwright2021quantitative}, showing that for each trail, pipe formation occurs every $\sim$100 kyr. \cite{cartwright2021quantitative} calculate that $\sim$30 MPa of overpressure is required for the initiation of venting at the Oceanus pipe trail from the Levant basin. Tectonic compression and marginal uplift have been proposed as the primary overpressuring mechanisms for episodic venting in the region \citep{cartwright2021quantitative, oppo2021leaky}. The Levant basin resides within a compressive tectonic regime stemming from the collision of the African and Eurasian plates. Here, we focus on 

